High-Order Langevin Diffusion Yields an Accelerated MCMC Algorithm

We propose a Markov chain Monte Carlo (MCMC) algorithm based on third-order Langevin dynamics for sampling from distributions with log-concave and smooth densities. The higher-order dynamics allow for more flexible discretization schemes, and we develop a specific method that combines splitting with more accurate integration. For a broad class of $d$-dimensional distributions arising from generalized linear models, we prove that the resulting third-order algorithm produces samples from a distribution that is at most $\varepsilon > 0$ in Wasserstein distance from the target distribution in $O\left(\frac{d^{1/4}}{ \varepsilon^{1/2}} \right)$ steps. This result requires only Lipschitz conditions on the gradient. For general strongly convex potentials with $\alpha$-th order smoothness, we prove that the mixing time scales as $O \left(\frac{d^{1/4}}{\varepsilon^{1/2}} + \frac{d^{1/2}}{\varepsilon^{1/(\alpha - 1)}} \right)$.

==> def.tex <==
\usepackage{caption}
\usepackage[utf8]{inputenc}

\usepackage{mathtools}
\usepackage{dsfont}
\usepackage{hyperref}
\usepackage{bm}
\usepackage{nicefrac}
\usepackage[dvipsnames]{xcolor}
\usepackage{wrapfig}
\usepackage{tikz}
\usepackage[colorinlistoftodos, textwidth=26mm, shadow,color=blue!30!white]{todonotes}
\usepackage{amsmath,amssymb,amsfonts,amsthm}
\usepackage{algorithmic}
%\usepackage[square, numbers]{natbib}
\usepackage[ruled,vlined]{algorithm2e}

\newcommand{\hmctransition}{\mathcal{T}}

\newcommand{\E}{\mathbb E}
\newcommand{\alg}{Rob-ULA\xspace}
\newcommand{\N}{\mathbb N}

\newcounter{assumption}%[section]
\renewcommand{\theassumption}{\arabic{assumption}}

\newenvironment{assumption}[1][]{\begin{trivlist}\item[] \refstepcounter{assumption}%
 {\bf{Assumption\ \theassumption\ }}{(#1)}.  }{%\par\nobreak\noindent\sl\ignorespaces}{%
 \ifvmode\smallskip\fi\end{trivlist}}

%Adding comments
\newcommand{\violet}[1]{\textcolor{red}{#1}}

%\newcommand{\R}{\mathbb{R}}
%\newcommand{\D}{\mathcal{D}}
\newcommand{\acc}{\varepsilon_{\textsf{acc}}}
\newcommand{\rd}{\mathrm{d}}
\newcommand{\ssh}{\hat{h}}
\newcommand{\lmx}{\lambda_{\text{max}}}
\newcommand{\lmn}{\lambda_{\text{min}}}
\newcommand{\eup}{\bar{\epsilon}}
\newcommand{\elo}{\underline{\epsilon}}
\newcommand\ip[2]{\langle #1, #2 \rangle}
\newcommand{\wtS}{\widetilde{\Sigma}}
\newcommand{\ex}{\mathbb{E}}
\newcommand{\lip}{L}
\newcommand{\conv}{m}
\newcommand{\cond}{\kappa}
\newcommand{\covsc}{\beta}
\newcommand{\wass}{\text{W}_2}
\newcommand{\convav}{\bar{\conv}}
\newcommand{\lipav}{\bar{\lip}}
\newcommand{\pari}{\tilde{\param}}
\newcommand*\Ep[1]{\mathbb{E}\left[#1\right]}
%\DeclareMathOperator*{\tr}{Tr}

\newcommand{\density}{p}
\newcommand{\initial}{p^0}
\newcommand{\target}{\ensuremath{p^*}}

\newcommand{\brackets}[1]{\left[ #1 \right]}
\newcommand{\parenth}[1]{\left( #1 \right)}
\newcommand{\bigparenth}[1]{\big( #1 \big)}
\newcommand{\biggparenth}[1]{\bigg( #1 \bigg)}
\newcommand{\braces}[1]{\left\{ #1 \right \}}
\newcommand{\abss}[1]{\left| #1 \right |}
\newcommand{\angles}[1]{\left\langle #1 \right \rangle}
\newcommand{\tp}{^\top}

\def\vx{{\bf x}}
\def\vX{{\bf X}}
\def\vy{{\bf y}}
\def\vz{{\bf z}}
\def\vv{{\bf v}}
\def\mD{{\rm D}}
\def\mQ{{\rm Q}}
\def\rd{\mathrm{d}}
\def\rT{{\rm T}}
\def\ball{\mathbb{B}}
\def\mI{\mathrm{I}}

\def\normal{\mathcal{N}}
\newcommand{\thetastar}{\theta_*}
\newcommand*{\p}{p}
\newcommand*{\q}{\mathbf{q}}
\newcommand*{\pmu}{\boldsymbol{\mu}}
\def\mI{\mathrm{I}}
%
%\newcommand{\matnorm}[3]{|\!|\!| #1 | \! | \!|_{{#2}, {#3}}}
%\newcommand{\matsnorm}[2]{|\!|\!| #1 | \! | \!|_{{#2}}}
%\newcommand{\vecnorm}[2]{\left\| #1\right\|_{#2}}
%\DeclarePairedDelimiterX{\infdivx}[2]{(}{)}{%
%  #1\;\delimsize\|\;#2%
%}
%\newcommand{\kldiv}{\text{KL}\infdivx}


\newcommand*\Mirr[1]{\textsc{Mirr} (#1)}
\newcommand*\Wd[0]{\textit{W}_2}
\newcommand*\dd[2]{\frac{\partial #1}{\partial #2}}
\newcommand*\stein[1]{\mathcal{A}_{#1}}
\newcommand*\w[0]{\textbf{w}}
\newcommand*\at[2]{\left.#1\right|_{#2}}
\newcommand*\ps[0]{p^*}
\newcommand*\del[0]{\partial}
\newcommand*\R[0]{\mathbb{R}}
\newcommand*\Z[0]{\mathbb{Z}}
\renewcommand*\div[0]{\nabla \cdot}
\newcommand*\ddt[0]{\frac{d}{d t}}
\newcommand*\dds[0]{\frac{d}{d s}}
\newcommand*\ddp[1]{\frac{\delta #1}{\delta p}}
\newcommand*\tr[0]{\text{tr}}
\newcommand*\KL[2]{\mathcal{KL}\left(#1\|#2\right)}
\newcommand*\lin[1]{\left\langle #1\right\rangle}
%\newcommand*\E[1]{\mathbb{E}\left[#1\right]}
%\newcommand*\Ep[2]{\mathbb{E}_{#1}\left[#2\right]}
%\newcommand*\grad[3]{\mathcal{D}_{#1}(#2,#3)}
\newcommand*\slope[1]{\|\mathcal{D}_{#1}\|}
\newcommand*\md[1]{\|\frac{d}{dt}#1\|}
\newcommand*\ap[2]{\tilde{#1}_{#2}}
\newcommand*\F[0]{\mathcal{F}}
\newcommand*\D[0]{\mathcal{D}}
\renewcommand*\H[0]{\mathcal{H}}
\newcommand*\G[0]{\mathcal{G}}
\newcommand*\Pspace[0]{\mathscr{P}}
\newcommand*\Uspace[0]{\mathbb{U}}
\renewcommand*\t[1]{\tilde{#1}}
\renewcommand*\d[0]{\delta}
\newcommand*\ot[1]{#1^{\perp}}
\newcommand*\proj[0]{\text{Proj}}
%\newcommand*{\qed}{\hfill\ensuremath{\square}}%
\newcommand\numberthis{\addtocounter{equation}{1}\tag{\theequation}}
\newcommand*\lrb[1]{\left[#1\right]}
\newcommand*\lrbb[1]{\left\{#1\right\}}
\newcommand*\lrp[1]{\left(#1\right)}
\newcommand*\lrn[1]{\left\|#1\right\|}
\newcommand*\eu[1]{\left\| #1\right\|}
\newcommand*\xt[0]{\tilde{x}}
\newcommand*\vt[0]{\tilde{v}}
\newcommand*\pt[0]{\tilde{p}}
\newcommand*\A[0]{\mathcal{A}}
\newcommand*\B[0]{\mathcal{B}}
\newcommand*\cvec[2]{\begin{bmatrix} #1\\#2\end{bmatrix}}
\newcommand*\bmat[1]{\begin{bmatrix} #1 \end{bmatrix}}
\newcommand*\pa[0]{\phi^\mathcal{A}}
\newcommand*\pb[0]{\phi^\mathcal{B}}
\newcommand*\Ts[0]{{T_{sync}}}
\newcommand*\tm[0]{{t^-}}
\newcommand*\ind[1]{{\mathds{1}\lrbb{#1}}}
\renewcommand*\proj[2]{{\Pi_{#1}\lrp{#2}}}
\renewcommand*{\tt}{{\tau(t)}}
\newcommand*{\ttm}{{\tau(\tm)}}
%\renewcommand*{\qed}{\hfill\ensuremath{\blacksquare}}
\renewcommand*{\Re}{\mathbb{R}}
\renewcommand*{\P}{\mathbf{P}}
\newcommand{\blank}[1]{\hfil\penalty1000\hfilneg\rule[-3pt]{#1}{0.4pt}} % nice blank underscores
%\newcommand*{\p}{\mathbf{p}}
% \newcommand*{\p}{p}
% \newcommand*{\q}{\mathbf{q}}
% \newcommand*{\pmu}{\boldsymbol{\mu}}
\def\mI{\mathrm{I}}

\def\vtheta{{{ \theta}}}
\def\dtheta{\Delta_\vtheta}
\def\vTheta{{{\Theta}}}
%\def\vzeta{{\bm{\zeta}}}
\def\vzeta{{{\zeta}}}
\def\vx{{\bf x}}
%\def\vX{{\bf X}}
\def\vX{\Theta}
\def\vy{{\bf y}}
\def\vz{{\bf z}}
\def\vv{{\bf v}}
\def\rd{\mathrm{d}}
\def\rT{{\rm T}}
\def\ball{\mathbb{B}}
\def\mI{\mathrm{I}}

%Numbering
\newcommand{\1}{\ensuremath{{\sf (i)}}}
\newcommand{\2}{\ensuremath{{\sf (ii)}}}
\newcommand{\3}{\ensuremath{{\sf (iii)}}}
\newcommand{\4}{\ensuremath{{\sf (iv)}}}
\newcommand{\5}{\ensuremath{{\sf (v)}}}
\newcommand{\6}{\ensuremath{{\sf (vi)}}}
\newcommand{\7}{\ensuremath{{\sf (vii)}}}
\newcommand{\8}{\ensuremath{{\sf (viii)}}}
\usepackage{amssymb}
%\newcommand*{\qed}{\hfill\ensuremath{\blacksquare}}%
\newcommand*{\Q}{\mathbf{Q}}
\newcommand*{\transpose}{\rm{T}}
\newcommand{\stepsize}{\eta}
\newcommand{\mya}[1]{\noindent{\textcolor{blue}{\{{\bf Yian:} \em #1\}}}}

\newcommand{\yccomment}[1]{\noindent{\textcolor{red}{\{{\bf Yuansi:} \em #1\}}}}

\newcommand{\mixingerror}{\epsilon}
\newcommand{\mixingtime}{\tau_{\text{mix}}}

\newcommand{\targetmeasure}{\mu}
\newcommand{\stationary}{\ensuremath{\Pi}}
\newcommand{\warmparam}{\beta}
\newcommand{\func}{U}
%\newcommand{\KL}{\text{KL}}
\newcommand{\proposal}{\mathcal{P}}


\newcommand{\step}{h}
\newcommand{\stepfunc}{w}
\newcommand{\stepbound}{\tilde{w}}
\newcommand{\scalar}{\alpha}
\newcommand{\tvscalar}{\gamma}


\newcommand{\transition}{\mathcal{T}}

\newcommand{\tagula}{\text{\tiny ULA}}
\newcommand{\tagmala}{\text{\tiny MALA}}
\newcommand{\tagmrw}{\text{\tiny MRW}}

\newcommand{\flow}{\phi}
\newcommand{\conductance}{\Phi}

\newcommand{\radius}{r}
\newcommand{\truncball}{\mathcal{R}}
\newcommand{\maxgrad}{\mathcal{D}}

\newcommand{\convexset}{\ensuremath{\mathcal{K}}}

\newcommand{\scparam}{m}
\newcommand{\smoothness}{L}
\newcommand{\condition}{\ensuremath{\kappa}}

\newcommand{\dims}{d}
\newcommand{\obs}{n}
\newcommand{\mydefn}{:=}
\newcommand{\logsobconstU}{\rho_U}
\newcommand{\logsobconst}{\rho}
\newcommand{\discretized}{\tilde}

\newcommand{\discStep}{\ensuremath{\left(t-k\stepsize\right)}}

\newcommand{\inprod}[2]{\ensuremath{\langle #1 , \, #2 \rangle}}
% Basic Math notations
\newcommand{\real}{\ensuremath{\mathbb{R}}}
\newcommand{\Ind}{\ensuremath{\mathbb{I}}}
% Probability
\newcommand{\Exs}{\ensuremath{{\mathbb{E}}}}
\newcommand{\Prob}{\ensuremath{{\mathbb{P}}}}

% % KL divergence
%\DeclarePairedDelimiterX{\infdivx}[2]{(}{)}{%
%  #1\;\delimsize\|\;#2%
%}
\newcommand{\kldiv}{\text{KL}\infdivx}


\newcommand{\NORMAL}{\ensuremath{\mathcal{N}}}
\newcommand{\BER}{\ensuremath{\mbox{Ber}}}

\newcommand{\Ot}{\tilde{\mathcal{O}}}
\newcommand{\Pc}{P}
\newcommand{\Pa}{Q}
% Brackets
\newcommand{\sphere}{\mathbb{S}}

% Some vector/matrix norms
\newcommand{\matnorm}[3]{|\!|\!| #1 | \! | \!|_{{#2}, {#3}}}
\newcommand{\matsnorm}[2]{|\!|\!| #1 | \! | \!|_{{#2}}}
\newcommand{\vecnorm}[2]{\left\| #1\right\|_{#2}}

\newcommand{\hessianlip}{L_2}
%%%%%%%%%%%%%%%%%%%%%%%%%%% Macros for the paper
\newcommand{\param}{\theta}
\newcommand{\Param}{\Theta}
\newcommand{\paramb}{\nu}
\newcommand{\data}{\mathcal{D}}
\newcommand{\z}{z}
\newcommand{\x}{x}
\newcommand{\prior}{p_\param}
\newcommand{\hyper}{\alpha}
\newcommand{\tfunc}{h}
\newcommand{\pmean}{q}
\newcommand{\f}{f}
\newcommand{\stp}{\eta}
\newcommand{\grad}{\nabla}
\newcommand{\gnoise}{\xi}
\newcommand{\lang}{\theta}
\newcommand{\g}{g}
\newcommand{\Cr}{C_{R}}
\newcommand{\Csa}{C_{\small{\Sigma, 1}}}
\newcommand{\Csb}{C_{\small{\Sigma, 2}}}
\newtheorem{lemma}{Lemma}
\newtheorem{theorem}{Theorem}
\newtheorem{corollary}{Corollary}
\newtheorem{proposition}{Proposition}
\newtheorem{remark}{Remark}
